Monads and limits in bicategories of circuits

We study monads in the (pseudo-)double category $\mathbf{KSW}(\mathcal{K})$ where loose arrows are Mealy automata valued in an ambient monoidal category $\mathcal{K}$, and the category of tight arrows is $\mathcal{K}$. Such monads turn out to be elegantly described through instances of semifree bicrossed products (bicrossed products of monoids, in the sense of Zappa-Sz\'ep-Takeuchi, where one factor is a free monoid). This result which gives an explicit description of the `free monad' double left adjoint to the forgetful functor. (Loose) monad maps are interesting as well, and relate to already known structures in automata theory. In parallel, we outline what double co/limits exist in $\mathbf{KSW}(\mathcal{K})$ and express in a synthetic language, based on double category theory, the bicategorical features of Katis-Sabadini-Walters `bicategory of circuits'.

==> secs/03-fib-2-dbl.tex <==
\section{From the universal fibration to the \PDC of Mealy automata, and back}\label{gnogni}
Recall from \cite{loregian2024automata} the following construction: given a category $\clK$, a diagram $B : \clB\to\clK$, and an endofunctor $F : \clK\to\clK$, the category of $F$-Mealy automata $\Mly(F,B)$ is obtained as follows:\footnote{A consequence of this description, which we will not exploit here but which will be the subject of future analysis, is that $\Mly(F,B)$ is the category of models of a $\Cat$-enriched sketch, in the sense of \cite{borceux1996enriched,borceux1998theory,Borceux2008}.}
\begin{itemize}
	\item take the \emph{inserter} $\Alg(F)$ of $F$ and $\id_\clK$, to build the object of $F$-algebras; then take the \emph{comma object} $F/B$;
	      % https://q.uiver.app/#q=WzAsNyxbMywwLCJGL0IiXSxbMiwxLCJcXGNsSyJdLFs0LDEsIlxcY2xCIl0sWzMsMiwiXFxjbEsiXSxbMSwyLCJcXGNsSyJdLFswLDEsIlxcY2xLIl0sWzEsMCwiXFxBbGcoRikiXSxbMCwxLCJWIiwyXSxbNiw1LCJVIiwyXSxbMSw0LCIiLDAseyJsZXZlbCI6Miwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsyLDMsIkIiXSxbNSw0LCJGIiwyXSxbNiwxLCJVIl0sWzEsMywiRiIsMl0sWzAsMiwiVSciXSxbMTEsOSwiIiwyLHsiY3VydmUiOi0yLCJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9fV0sWzEzLDEwLCIiLDEseyJjdXJ2ZSI6LTIsInNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH19XV0=
	      \[\begin{tikzcd}[cramped,sep=small]
			      & {\Alg(F)} && {F/B} \\
			      \clK && \clK && \clB \\
			      & \clK && \clK
			      \arrow["U"', from=1-2, to=2-1]
			      \arrow["U", from=1-2, to=2-3]
			      \arrow["V"', from=1-4, to=2-3]
			      \arrow["{U'}", from=1-4, to=2-5]
			      \arrow[""{name=0, anchor=center, inner sep=0}, "F"', from=2-1, to=3-2]
			      \arrow[""{name=1, anchor=center, inner sep=0}, Rightarrow, no head, from=2-3, to=3-2]
			      \arrow[""{name=2, anchor=center, inner sep=0}, "F"', from=2-3, to=3-4]
			      \arrow[""{name=3, anchor=center, inner sep=0}, "B", from=2-5, to=3-4]
			      %\arrow[bend left=40, shorten <=8pt, shorten >=8pt, Rightarrow, from=0, to=1]
			      %\arrow[bend left=30, shorten <=10pt, shorten >=10pt, Rightarrow, from=2, to=3]
		      \end{tikzcd}\]
	\item now take the strict pullback of the cospan $U,V$; this is $\Mly(F,B)$, which now has been defined in a fashion that suits to any 2-category with finite limits.

	      The objects and morphisms of $\Mly(F,B)$ are, respectively, obtained as spans $\langle X,Y,d,s\rangle : X \xot d FX \xto s BY$ and pairs $u,v$ of morphisms in $\clK$ such that the squares in
	      % https://q.uiver.app/#q=WzAsNixbMSwwLCJGWCJdLFswLDAsIlgiXSxbMSwxLCJGWCciXSxbMCwxLCJYJyJdLFsyLDAsIkJZIl0sWzIsMSwiQlknIl0sWzAsNCwicyJdLFswLDEsImQiLDJdLFsyLDMsImQnIiwyXSxbMiw1LCJzJyJdLFswLDIsIkZ1IiwyXSxbNCw1LCJCdiJdLFsxLDMsInUiLDJdXQ==
	      \[\begin{tikzcd}[cramped]
			      X & FX & BY \\
			      {X'} & {FX'} & {BY'}
			      \arrow["u"', from=1-1, to=2-1]
			      \arrow["d"', from=1-2, to=1-1]
			      \arrow["s", from=1-2, to=1-3]
			      \arrow["Fu"', from=1-2, to=2-2]
			      \arrow["Bv", from=1-3, to=2-3]
			      \arrow["{d'}"', from=2-2, to=2-1]
			      \arrow["{s'}", from=2-2, to=2-3]
		      \end{tikzcd}\]
	      both commute.
\end{itemize}
In particular, when $\clK$ is Cartesian, $B : 1\to\clK$ is an object of $\clK$, and $F = A\times\_$ is the functor `product by $A\in\clK$', we get back the category $\Mly(A,B)$ whose objects are spans like \eqref{florpo}. This can be conveniently packaged in the presence of a pseudofunctor
% https://q.uiver.app/#q=WzAsMixbMCwwLCJcXE1seTpcXGNsS15cXG9wXFx0aW1lc1xcY2xLIl0sWzIsMCwiXFxDYXQiXSxbMCwxXV0=
\[\begin{tikzcd}[cramped]
		{\Mly:\clK^\op\times\clK} & \Cat
		\arrow[from=1-1, to=1-2]
	\end{tikzcd}\]
in turn giving rise to a split Grothendieck fibration over $\clK^\op\times\clK$ called the \emph{universal Mealy fibration} in \cite{loregian2024automata}. In this section we describe the relation in which the universal Mealy fibration $\Mly$ and the \PDC $\dblMly$ built in \autoref{def_dbl_processes} stand.

% \begin{center}
% \includegraphics[width=\textwidth]{one.jpg}

% \includegraphics[width=\textwidth]{two.jpg}

% \includegraphics[width=\textwidth]{tre.jpg}
% \end{center}
The idea is to exploit the result of \cite{lawler2015fibrationspredicatesbicategoriesrelations}, where it is hown that the following pieces of data are equivalent:
\begin{itemize}
	\item a $\Cat$-enriched promonad $M : \clK^\op\times\clK\to\Cat$, i.e. a pseudofunctor so that, regarded as a pseudoprofunctor $\clK\pro \clK$, satisfies the axioms of a pseudomonad inside the 3-category of 2-categories, pseudoprofunctors, and pseudoprofunctor 2- and 3-cells.
	\item A double category $\dblCat{D}$ admitting all companions.
\end{itemize}
This construction makes the functor $\dblCat{D}_t \to \dblCat{D}_\ell$ sending a tight 1-cell to its companion a proarrow equipment; the loose bicategory $\dblCat{D}_\ell$ boils down to be the Kleisli bicategory of such an identity-on-objects map.



==> secs/04-future.tex <==
\section{Future work}
In the case of a non-Cartesian monoidal category $\clK$ of processes some aspects of the theory get more interesting;
there are nonCartesian cases where the monoidal structure is still manageable and retains some intuition, e.g. the semiCartesian case given by the Kleisli category of a probability monad \cite{Fritz2020,Jacobs2018,Doberkat2007,Fritz2023}. It would be interesting to study the semiCartesian \PDC of probabilistic Mealy automata.

Monads also become more interesting, and comonads nontrivial, in situations where the monoidal structure is canonical enough (e.g. when $\clK$ is the category of $R$-modules, or a category of representations of a groupoid like in \cite{loregian2024automata}).

The co/completeness properties of $\cartDblMly$ make it a strange animal: tight colimit fail to exist for a silly reason; tight limits exist and are induced by $\clK$, but \emph{double} limits fail to exist due to the absence of tabulators. The existence of some universal objects, like Kan extensions, Kan lifts, and co/comma objects might be interesting to rule out or characterize.

The search for co/completeness theorems is not only motivated by purely category-theoretic interest; often, we can give computational meaning to universal properties, and constructions that are nicely described in the bicategory probably acquire a better description in the double category: for example, behaviour as Kan extension \cite{Bainbridge1975}, or minimization in the sense of \cite{lmcs_6213}.

Tackling the former problem goes in the direction of further generalization: in \cite{Grandis2019} the authors define an \emph{internal hom} double category $\dblCat{[C,D]}$ in the category of \PDC{s} (the definition is space consuming and it is recalled below, cf. \autoref{exp_o_dbl}); replacing Walters' bicategory with the double category of pseudo double functors $\bbN \to \dblMly$ should lead to some insight about the universal properties it has \emph{qua} \PDC.

==> secs/05-paralipomena.tex <==
\section{Paralipomena and proofs}
\begin{definition}[\PDC]\label{def_pdc}
	A \emph{\PDC} consists of
	\begin{enumerate}
		\item \label{def_dbl_1} a class of objects $X,Y,Z,\dots$;
		\item \label{def_dbl_2} a category $\clD_0$ of \emph{tight morphisms};
		\item \label{def_dbl_3} for every pair of objects $X,Y$ a set of \emph{loose morphisms} $p : X\pto Y$;
		\item \label{def_dbl_4} for every quadruple of tight and loose morphisms sharing boundary objects as in
		      % https://q.uiver.app/#q=WzAsNCxbMCwwLCJYIl0sWzEsMCwiWSJdLFswLDEsIloiXSxbMSwxLCJXIl0sWzAsMiwiZiIsMl0sWzEsMywiZyJdLFswLDEsInAiLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbMiwzLCJxIiwyLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fV0sWzYsNywiXFxhbHBoYSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==
		      \[\begin{tikzcd}[cramped]
				      X & Y \\
				      Z & W
				      \arrow[""{name=0, anchor=center, inner sep=0}, "p", "\shortmid"{marking}, from=1-1, to=1-2]
				      \arrow["f"', from=1-1, to=2-1]
				      \arrow["g", from=1-2, to=2-2]
				      \arrow[""{name=1, anchor=center, inner sep=0}, "q"', "\shortmid"{marking}, from=2-1, to=2-2]
			      \end{tikzcd}\]
		      a set of \emph{cells} $\alpha$ having $p$ as \emph{loose domain}, $q$ as \emph{loose codomain}, $f$ as \emph{tight domain}, $g$ as \emph{tight codomain};
		\item \label{def_dbl_5} distinguished loose morphisms denoted $i_X : \idpto X$, and distinguished cells
		      % https://q.uiver.app/#q=WzAsNCxbMCwwLCJBIl0sWzEsMCwiQSJdLFswLDEsIkIiXSxbMSwxLCJCIl0sWzAsMiwiZiIsMl0sWzEsMywiZiJdLFswLDEsImlfQSIsMCx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFsyLDMsImlfQiIsMix7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFswLDMsImlfZiIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==
		      \[\begin{tikzcd}[cramped]
				      A & A \\
				      B & B
				      \arrow["{i_A}",Rightarrow, no head,  "\shortmid"{marking}, from=1-1, to=1-2]
				      \arrow["f"', from=1-1, to=2-1]
				      \arrow["{\iota_f}"{description}, draw=none, from=1-1, to=2-2]
				      \arrow["f", from=1-2, to=2-2]
				      \arrow["{i_B}"', Rightarrow, no head, "\shortmid"{marking}, from=2-1, to=2-2]
			      \end{tikzcd}\]
		      for every tight morphism $f : A \to B$, and distinguished cells
		      % https://q.uiver.app/#q=WzAsNCxbMCwwLCJYIl0sWzEsMCwiWSJdLFswLDEsIlgiXSxbMSwxLCJZIl0sWzAsMSwicCIsMCx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFsyLDMsInAiLDIseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbMCwyLCIiLDIseyJsZXZlbCI6Miwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxLDMsIiIsMCx7ImxldmVsIjoyLCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzAsMywiXFxpb3RhX3AiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XV0=
		      \[\begin{tikzcd}[cramped]
				      X & Y \\
				      X & Y
				      \arrow["p", "\shortmid"{marking}, from=1-1, to=1-2]
				      \arrow[Rightarrow, no head, from=1-1, to=2-1]
				      \arrow["{\iota_p}"{description}, draw=none, from=1-1, to=2-2]
				      \arrow[Rightarrow, no head, from=1-2, to=2-2]
				      \arrow["p"', "\shortmid"{marking}, from=2-1, to=2-2]
			      \end{tikzcd}\]
		      for every loose morphism $p : X\to Y$ (where vertically we put the identities of $X,Y$ in the category $\clD_0$);
		\item \label{def_dbl_6} composition laws for cells, along the loose direction,
		      % https://q.uiver.app/#q=WzAsMTAsWzAsMCwiWCJdLFsxLDAsIlkiXSxbMiwwLCJaIl0sWzAsMSwiWCciXSxbMSwxLCJZJyJdLFsyLDEsIlonIl0sWzQsMCwiWCJdLFs1LDAsIloiXSxbNCwxLCJYJyJdLFs1LDEsIlonIl0sWzAsMywiZiIsMl0sWzEsNCwiZyIsMl0sWzIsNSwiaCJdLFswLDEsInAiLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbMSwyLCJwJyIsMCx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFszLDQsInEiLDIseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbNCw1LCJxJyIsMix7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFsyLDgsIlxcbWFwc3RvIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzYsOCwiZiIsMl0sWzcsOSwiaCJdLFs2LDcsInAnXFxob3JDIHAiLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbOCw5LCJxJ1xcaG9yQyBxIiwyLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fV0sWzAsNCwiXFxhbHBoYSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxLDUsIlxcYmV0YSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs2LDksIlxcYmV0YVxcaG9yQ1xcYWxwaGEiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XV0=
		      \[\begin{tikzcd}[cramped]
				      X & Y & Z && X & Z \\
				      {X'} & {Y'} & {Z'} && {X'} & {Z'}
				      \arrow["p", "\shortmid"{marking}, from=1-1, to=1-2]
				      \arrow["f"', from=1-1, to=2-1]
				      \arrow["\alpha"{description}, draw=none, from=1-1, to=2-2]
				      \arrow["{p'}", "\shortmid"{marking}, from=1-2, to=1-3]
				      \arrow["g"', from=1-2, to=2-2]
				      \arrow["\beta"{description}, draw=none, from=1-2, to=2-3]
				      \arrow["h", from=1-3, to=2-3]
				      \arrow["\mapsto"{description}, draw=none, from=1-3, to=2-5]
				      \arrow["{p'\horC p}", "\shortmid"{marking}, from=1-5, to=1-6]
				      \arrow["f"', from=1-5, to=2-5]
				      \arrow["{\beta\horC\alpha}"{description}, draw=none, from=1-5, to=2-6]
				      \arrow["h", from=1-6, to=2-6]
				      \arrow["q"', "\shortmid"{marking}, from=2-1, to=2-2]
				      \arrow["{q'}"', "\shortmid"{marking}, from=2-2, to=2-3]
				      \arrow["{q'\horC q}"', "\shortmid"{marking}, from=2-5, to=2-6]
			      \end{tikzcd}\]
		      and along the tight direction, here prescribed according to the category structure on $\clD_0$:
		      % https://q.uiver.app/#q=WzAsMTAsWzAsMCwiWCJdLFsxLDAsIkEiXSxbMCwxLCJZIl0sWzEsMSwiQiJdLFswLDIsIloiXSxbMSwyLCJDIl0sWzMsMCwiWCJdLFszLDIsIloiXSxbNCwwLCJBIl0sWzQsMiwiQyJdLFswLDIsImYiLDJdLFsxLDMsImciXSxbMCwxLCJwIiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fV0sWzIsMywicSIsMix7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFswLDMsIlxcYWxwaGEiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMiw0LCJmJyIsMl0sWzMsNSwiZyciXSxbNCw1LCJyIiwyLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fV0sWzIsNSwiXFxiZXRhIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzYsNywiZidmIiwyXSxbOCw5LCJnJ2ciXSxbNiw4LCJwIiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fV0sWzcsOSwiciIsMix7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFs2LDksIlxcYmV0YVxcdmVyQ1xcYWxwaGEiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMSw3LCJcXG1hcHN0byIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==
		      \[\begin{tikzcd}[row sep=4mm,cramped]
				      X & A && X & A \\
				      Y & B \\
				      Z & C && Z & C
				      \arrow["p", "\shortmid"{marking}, from=1-1, to=1-2]
				      \arrow["f"', from=1-1, to=2-1]
				      \arrow["\alpha"{description}, draw=none, from=1-1, to=2-2]
				      \arrow["g", from=1-2, to=2-2]
				      \arrow["\mapsto"{description}, draw=none, from=1-2, to=3-4]
				      \arrow["p", "\shortmid"{marking}, from=1-4, to=1-5]
				      \arrow["{f'f}"', from=1-4, to=3-4]
				      \arrow["{\beta\vertC\alpha}"{description}, draw=none, from=1-4, to=3-5]
				      \arrow["{g'g}", from=1-5, to=3-5]
				      \arrow["q"', "\shortmid"{marking}, from=2-1, to=2-2]
				      \arrow["{f'}"', from=2-1, to=3-1]
				      \arrow["\beta"{description}, draw=none, from=2-1, to=3-2]
				      \arrow["{g'}", from=2-2, to=3-2]
				      \arrow["r"', "\shortmid"{marking}, from=3-1, to=3-2]
				      \arrow["r"', "\shortmid"{marking}, from=3-4, to=3-5]
			      \end{tikzcd}\]
		\item \label{def_dbl_7} \emph{associator} and \emph{unitor} invertible cells
		      % https://q.uiver.app/#q=WzAsMTYsWzAsMCwiWCJdLFsyLDAsIloiXSxbMCwxLCJYIl0sWzEsMSwiWSJdLFszLDAsIlciXSxbMywxLCJXIl0sWzQsMCwiWCJdLFs1LDAsIlkiXSxbNiwwLCJZIl0sWzQsMSwiWCJdLFs2LDEsIlkiXSxbNywwLCJYIl0sWzgsMCwiWCJdLFs5LDAsIlkiXSxbNywxLCJYIl0sWzksMSwiWSJdLFsyLDMsInIiLDIseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbMyw1LCJwXFxob3JDIHEiLDIseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbMCwxLCJxXFxob3JDIHIiLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbMSw0LCJwIiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fV0sWzAsMiwiIiwxLHsibGV2ZWwiOjIsInN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNCw1LCIiLDEseyJsZXZlbCI6Miwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFswLDUsIlxcdGV4dHthc3NvY30iLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNiw3LCJwIiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fV0sWzcsOCwiaV9ZIiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fV0sWzksMTAsInAiLDIseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbMTQsMTUsInAiLDIseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbMTEsMTIsImlfWCIsMCx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFsxMiwxMywicCIsMCx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFs2LDksIiIsMix7ImxldmVsIjoyLCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzgsMTAsIiIsMCx7ImxldmVsIjoyLCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzExLDE0LCIiLDIseyJsZXZlbCI6Miwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxMywxNSwiIiwwLHsibGV2ZWwiOjIsInN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNiwxMCwiXFx0ZXh0e3VuaXR9XkwiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTEsMTUsIlxcdGV4dHt1bml0fV5SIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
		      \[\begin{tikzcd}[cramped]
				      X && Z & W & X & Y & Y & X & X & Y \\
				      X & Y && W & X && Y & X && Y.
				      \arrow["{q\horC r}", "\shortmid"{marking}, from=1-1, to=1-3]
				      \arrow[Rightarrow, no head, from=1-1, to=2-1]
				      \arrow["{\mathrm{assoc}}"{description}, draw=none, from=1-1, to=2-4]
				      \arrow["p", "\shortmid"{marking}, from=1-3, to=1-4]
				      \arrow[Rightarrow, no head, from=1-4, to=2-4]
				      \arrow["p", "\shortmid"{marking}, from=1-5, to=1-6]
				      \arrow[Rightarrow, no head, from=1-5, to=2-5]
				      \arrow["{\mathrm{unit}^L}"{description}, draw=none, from=1-5, to=2-7]
				      \arrow["{i_Y}", "\shortmid"{marking}, from=1-6, to=1-7]
				      \arrow[Rightarrow, no head, from=1-7, to=2-7]
				      \arrow["{i_X}", "\shortmid"{marking}, from=1-8, to=1-9]
				      \arrow[Rightarrow, no head, from=1-8, to=2-8]
				      \arrow["{\mathrm{unit}^R}"{description}, draw=none, from=1-8, to=2-10]
				      \arrow["p", "\shortmid"{marking}, from=1-9, to=1-10]
				      \arrow[Rightarrow, no head, from=1-10, to=2-10]
				      \arrow["r"', "\shortmid"{marking}, from=2-1, to=2-2]
				      \arrow["{p\horC q}"', "\shortmid"{marking}, from=2-2, to=2-4]
				      \arrow["p"', "\shortmid"{marking}, from=2-5, to=2-7]
				      \arrow["p"', "\shortmid"{marking}, from=2-8, to=2-10]
			      \end{tikzcd}\]
	\end{enumerate}
	All these data are subject to the conditions stated in \cite[§7.1]{Grandis1999}, particularly, [\emph{ibi}, pdc2.1---pdc2.6]:
	\begin{enumerate}%{da}
		\item \label{da_1} (weak) associativity of loose composition: given composable cells $\alpha,\beta,\gamma$ the two possible loose compositions $\alpha\mid \gamma\horC\beta$ and $\beta\horC\alpha\mid\gamma$;
		      differ by the associator in \autoref{def_dbl_7};
		\item \label{da_2} (weak) unitality of loose composition;
		\item \label{da_2'} (weak) associativity of loose composition;
		\item bicategory axioms (pentagon and triangle) for loose composition;
		\item \label{da_3} axioms of category for the tight composition;
		\item \label{da_4} interchange law.
	\end{enumerate}
	% \todo[inline]{}
\end{definition}
The adjective `weak' is what qualifies the resulting structure as a \emph{pseudo} double category. One situation when a double category arises naturally is when a category $\clC$ is given, together with a bicategory having the same objects and a natural choice of cells as in \eqref{baiadiai}. This is for example the case of the double category of modules, cf. \cite[Example 2.2]{Shulman2008a}, the more general double category of distributors, and the double category of relations in a regular category, cf. \cite{dawson2010span} and \cite{Freyd1990}.
\begin{definition}[Duals of a \PDC]\label{los_duales}
	There are three notions of dual for a \PDC $\dblD$:
	\begin{itemize}
		\item the loose dual $\dblD^\hop$ defined reversing the direction of the loose morphisms;
		\item the tight dual $\dblD^\vop$ defined reversing the direction of the tight morphisms;
		\item the double dual $\dblD^\oop$ defined reversing the direction of both loose and tight morphisms.
	\end{itemize}
	% \todo[inline]{check if the latter concides with `reversing cells'?}
\end{definition}
\begin{definition}
	The cotabulator of a loose morphism $F : A\pto B$ in a \PDC $\dblD$ consists of a pair $(\cotabu F, \tau_F)$ where $\cotabu F$ is an object of $\dblD$, and $\tau_F$ a cell
	% https://q.uiver.app/#q=WzAsNCxbMCwwLCJBIl0sWzEsMCwiQiJdLFswLDEsIlxcdGF1XlxcY2lyYyBGIl0sWzEsMSwiXFx0YXVeXFxjaXJjIEYiXSxbMCwxLCJGIiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fV0sWzIsMywiIiwwLHsibGV2ZWwiOjIsInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzAsMiwiYSIsMl0sWzEsMywiYiJdLFswLDMsIlxcdGF1IEYiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XV0=
	$\begin{tikzcd}[cramped]
			A & B \\
			{\cotabu F} & {\cotabu F}
			\arrow["F", "\shortmid"{marking}, from=1-1, to=1-2]
			\arrow["a"', from=1-1, to=2-1]
			\arrow["{\tau_F}"{description}, draw=none, from=1-1, to=2-2]
			\arrow["b", from=1-2, to=2-2]
			\arrow["\shortmid"{marking}, Rightarrow, no head, from=2-1, to=2-2]
		\end{tikzcd}$
	universal among all such, i.e. with the property that any other cell
	% https://q.uiver.app/#q=WzAsNCxbMCwwLCJBIl0sWzEsMCwiQiJdLFswLDEsIlgiXSxbMSwxLCJYIl0sWzAsMSwiRiIsMCx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFsyLDMsIiIsMCx7ImxldmVsIjoyLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFswLDIsInAiLDJdLFsxLDMsInEiXSxbMCwzLCJcXHhpIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
	$\begin{tikzcd}[cramped]
			A & B \\
			X & X
			\arrow["F", "\shortmid"{marking}, from=1-1, to=1-2]
			\arrow["p"', from=1-1, to=2-1]
			\arrow["\xi"{description}, draw=none, from=1-1, to=2-2]
			\arrow["q", from=1-2, to=2-2]
			\arrow["\shortmid"{marking}, Rightarrow, no head, from=2-1, to=2-2]
		\end{tikzcd}$
	factors uniquely through $\tau_F$ as
	% https://q.uiver.app/#q=WzAsMTAsWzAsMCwiQSJdLFsxLDAsIkIiXSxbMCwyLCJYIl0sWzEsMiwiWCJdLFsyLDAsIkEiXSxbMywwLCJCIl0sWzIsMSwiXFxjb3RhYnUgRiJdLFszLDEsIlxcY290YWJ1IEYiXSxbMiwyLCJYIl0sWzMsMiwiWCJdLFswLDEsIkYiLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbMiwzLCIiLDAseyJsZXZlbCI6Miwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMCwyLCJwIiwyXSxbMSwzLCJxIl0sWzAsMywiXFx4aSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs0LDUsIkYiLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbNCw2XSxbNiw4XSxbNSw3XSxbNyw5XSxbOCw5LCIiLDIseyJsZXZlbCI6Miwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNiw3LCIiLDEseyJsZXZlbCI6Miwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNiw5LCJcXGhhdFxceGkiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNCw3LCJcXHRhdV9GIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
	\[\label{cotab_univ}\begin{tikzcd}[row sep=4mm,cramped]
			A & B & A & B \\
			&& {\cotabu F} & {\cotabu F} \\
			X & X & X & X
			\arrow["F", "\shortmid"{marking}, from=1-1, to=1-2]
			\arrow["p"', from=1-1, to=3-1]
			\arrow["\xi"{description}, draw=none, from=1-1, to=3-2]
			\arrow["q", from=1-2, to=3-2]
			\arrow["{=}"{description}, draw=none, from=1-2, to=3-3]
			\arrow["F", "\shortmid"{marking}, from=1-3, to=1-4]
			\arrow[from=1-3, to=2-3]
			\arrow["{\tau_F}"{description}, draw=none, from=1-3, to=2-4]
			\arrow[from=1-4, to=2-4]
			\arrow["\shortmid"{marking}, Rightarrow, no head, from=2-3, to=2-4]
			\arrow[from=2-3, to=3-3]
			\arrow["{\hat\xi}"{description}, draw=none, from=2-3, to=3-4]
			\arrow[from=2-4, to=3-4]
			\arrow["\shortmid"{marking}, Rightarrow, no head, from=3-1, to=3-2]
			\arrow["\shortmid"{marking}, Rightarrow, no head, from=3-3, to=3-4]
		\end{tikzcd}\]
\end{definition}
The \emph{tabulator} of a loose morphism $F : A\pto B$ is defined as the cotabulator of $F$ in $\dblD^\vop$, and it consists of a universal cell
% https://q.uiver.app/#q=WzAsNCxbMCwxLCJBIl0sWzEsMSwiQiJdLFswLDAsIlxcdGFidSBGIl0sWzEsMCwiXFx0YWJ1IEYiXSxbMCwxLCJGIiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fV0sWzIsMywiIiwwLHsibGV2ZWwiOjIsInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzIsMCwiYSIsMl0sWzMsMSwiYiJdLFswLDMsIlxcdmFycGkgRiIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==
$\begin{tikzcd}[cramped]
		{\tabu F} & {\tabu F} \\
		A & B
		\arrow["\shortmid"{marking}, Rightarrow, no head, from=1-1, to=1-2]
		\arrow["a"', from=1-1, to=2-1]
		\arrow["b", from=1-2, to=2-2]
		\arrow["{\varpi_F}"{description}, draw=none, from=2-1, to=1-2]
		\arrow["F", "\shortmid"{marking}, from=2-1, to=2-2]
	\end{tikzcd}$
subject to the dual universal property of\eqref{cotab_univ}.

In the following definitions we outline the notion of (tight) co/limit in a \PDC $\dblD$, drawing from \cite[§4.2]{Grandis1999}. We do not need to describe colimits explicitly, as they seldom exist in $\cartDblMly$, so we are content with the tautological definition of `limits in the vertical dual of $\dblD$'.
\begin{definition}[Initial and terminal objects in a \PDC]\label{def_initerm_pc}
	A \emph{terminal object} in $\dblD$ consists of an object $\top$ which is terminal in the tight category $\clD_0$, and such that for every loose morphism $p : A\pto B$ there is a unique cell
	\[\begin{tikzcd}
			A \ar[d, "!_A"']\ar[r, "\shortmid"{marking}, "p"] & B\ar[d, "!_B"]\\
			\top \ar[r, "\shortmid"{marking}, Rightarrow,no head]& \top .
			\arrow["{!_p}"{description}, draw=none, from=1-1, to=2-2]
		\end{tikzcd}\]
	Dually, an initial object in $\dblD$ consists of a terminal object in $\dblD^\vop$.
\end{definition}
(Generalizing the following definition to the case of a family $(A_i\mid i\in I)$ of objects is straightforward.)
\begin{definition}[Products and coproducts in a \PDC]\label{def_procopro_pc}
	Let $A,B$ be two objects of $\dblD$; the \emph{double product} $A\times B$ of the two objects consists of a pair of cells
	% https://q.uiver.app/#q=WzAsOCxbMCwwLCJBXFx0aW1lcyBCIl0sWzAsMSwiQSJdLFsxLDEsIkEiXSxbMSwwLCJBXFx0aW1lcyBCIl0sWzIsMCwiQVxcdGltZXMgQiJdLFszLDAsIkFcXHRpbWVzIEIiXSxbMiwxLCJCIl0sWzMsMSwiQiJdLFswLDEsInBfQSIsMl0sWzMsMiwicF9BIl0sWzQsNiwicF9CIiwyXSxbNSw3LCJwX0IiXSxbMCwzLCIiLDEseyJsZXZlbCI6Miwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMSwyLCIiLDEseyJsZXZlbCI6Miwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNCw1LCIiLDEseyJsZXZlbCI6Miwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNiw3LCIiLDEseyJsZXZlbCI6Miwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMCwyLCJcXHBpX0EiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNCw3LCJcXHBpX0IiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XV0=
	\[\begin{tikzcd}[cramped]
			{A\times B} & {A\times B} & {A\times B} & {A\times B} \\
			A & A & B & B
			\arrow["\shortmid"{marking}, Rightarrow, no head, from=1-1, to=1-2]
			\arrow["{p_A}"', from=1-1, to=2-1]
			\arrow["{\pi_A}"{description}, draw=none, from=1-1, to=2-2]
			\arrow["{p_A}", from=1-2, to=2-2]
			\arrow["\shortmid"{marking}, Rightarrow, no head, from=1-3, to=1-4]
			\arrow["{p_B}"', from=1-3, to=2-3]
			\arrow["{\pi_B}"{description}, draw=none, from=1-3, to=2-4]
			\arrow["{p_B}", from=1-4, to=2-4]
			\arrow["\shortmid"{marking}, Rightarrow, no head, from=2-1, to=2-2]
			\arrow["\shortmid"{marking}, Rightarrow, no head, from=2-3, to=2-4]
		\end{tikzcd}\]
	that are universal in the following sense: given any loose morphism $u : X\pto Y$, tight morphisms $A \xot a X \xto b B$ and $A \xot {a'} Y \xto {b'} B$ and cells
	% https://q.uiver.app/#q=WzAsOCxbMCwwLCJYIl0sWzEsMCwiWSJdLFswLDEsIkEiXSxbMSwxLCJBIl0sWzIsMCwiWCJdLFszLDAsIlkiXSxbMiwxLCJCIl0sWzMsMSwiQiJdLFswLDEsInUiLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbMCwyLCJhIiwyXSxbMSwzLCJhJyJdLFsyLDMsIiIsMix7ImxldmVsIjoyLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs0LDUsInUiLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbNiw3LCIiLDIseyJsZXZlbCI6Miwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNCw2LCJiIiwyXSxbNSw3LCJiJyJdLFswLDMsIlxceGlfMSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs0LDcsIlxceGlfMiIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==
	\[\begin{tikzcd}[cramped]
			X & Y & X & Y \\
			A & A & B & B
			\arrow["u", "\shortmid"{marking}, from=1-1, to=1-2]
			\arrow["a"', from=1-1, to=2-1]
			\arrow["{\xi_1}"{description}, draw=none, from=1-1, to=2-2]
			\arrow["{a'}", from=1-2, to=2-2]
			\arrow["u", "\shortmid"{marking}, from=1-3, to=1-4]
			\arrow["b"', from=1-3, to=2-3]
			\arrow["{\xi_2}"{description}, draw=none, from=1-3, to=2-4]
			\arrow["{b'}", from=1-4, to=2-4]
			\arrow["\shortmid"{marking}, Rightarrow, no head, from=2-1, to=2-2]
			\arrow["\shortmid"{marking}, Rightarrow, no head, from=2-3, to=2-4]
		\end{tikzcd}\]
	\begin{enumerate}
		\item there exists a unique pair of tight morphisms $\langle a,b\rangle : X\to A\times B$ and $\langle a',b'\rangle : Y\to A\times B$ so that the tuple $(A\times B; p_A,p_B)$ is a product in $\clD_0$ (so, in particular, $p_A\circ\langle a,b\rangle = a$, $p_B\circ \langle a,b\rangle = b$, $p_A\circ \langle a',b'\rangle = a'$, $p_B\circ \langle a',b'\rangle = b'$);
		\item there exists a unique cell
		      % https://q.uiver.app/#q=WzAsNCxbMCwwLCJYIl0sWzEsMCwiWSJdLFswLDEsIkFcXHRpbWVzIEIiXSxbMSwxLCJBXFx0aW1lcyBCIl0sWzAsMSwidSIsMCx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFswLDIsIlxcbGFuZ2xlIGEsYlxccmFuZ2xlIiwyXSxbMSwzLCJcXGxhbmdsZSBhJyxiJ1xccmFuZ2xlIl0sWzIsMywiIiwyLHsibGV2ZWwiOjIsInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzAsMywiXFxsYW5nbGVcXHhpXzEsXFx4aV8yXFxyYW5nbGUiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XV0=
		      \[\begin{tikzcd}[cramped]
				      X & Y \\
				      {A\times B} & {A\times B}
				      \arrow["u", "\shortmid"{marking}, from=1-1, to=1-2]
				      \arrow["{\langle a,b\rangle}"', from=1-1, to=2-1]
				      \arrow["{\langle\xi_1,\xi_2\rangle}"{description}, draw=none, from=1-1, to=2-2]
				      \arrow["{\langle a',b'\rangle}", from=1-2, to=2-2]
				      \arrow["\shortmid"{marking}, Rightarrow, no head, from=2-1, to=2-2]
			      \end{tikzcd}\]
		      such that the equalities of cells $\xi_1 = \frac{\langle \xi_1,\xi_2\rangle}{\pi_A}$ and $\xi_2 = \frac{\langle \xi_1,\xi_2\rangle}{\pi_B}$ hold.
	\end{enumerate}
	The \emph{double coproduct} of $A, B$ consists of the double product of $A,B$ in $\dblD^\vop$.
\end{definition}
\begin{definition}[Pullbacks and pushouts in a \PDC]\label{def_pullpush_pc}
	Let $A \xto f X \xot g B$ be a cospan of tight morphisms in $\dblD$; the \emph{double pullback} of $f,g$ in $\dblD$ consists of an arrangement of cells
	% https://q.uiver.app/#q=WzAsOCxbMCwwLCJBXFx0aW1lc19YIEIiXSxbMSwwLCJBXFx0aW1lc19YIEIiXSxbMCwxLCJBIl0sWzEsMSwiQSJdLFsyLDAsIkFcXHRpbWVzX1ggQiJdLFszLDAsIkFcXHRpbWVzX1ggQiJdLFsyLDEsIkIiXSxbMywxLCJCIl0sWzAsMiwicF9BIiwyXSxbMSwzLCJwX0EiXSxbNCw2LCJwX0IiLDJdLFs1LDcsInBfQiJdLFswLDEsIiIsMSx7ImxldmVsIjoyLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsyLDMsIiIsMSx7ImxldmVsIjoyLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs0LDUsIiIsMSx7ImxldmVsIjoyLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs2LDcsIiIsMSx7ImxldmVsIjoyLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFswLDMsIlxccGlfQSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs0LDcsIlxccGlfQiIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==
	\[\begin{tikzcd}[cramped]
			{A\times_X B} & {A\times_X B} & {A\times_X B} & {A\times_X B} \\
			A & A & B & B
			\arrow["\shortmid"{marking}, Rightarrow, no head, from=1-1, to=1-2]
			\arrow["{p_A}"', from=1-1, to=2-1]
			\arrow["{\pi_A}"{description}, draw=none, from=1-1, to=2-2]
			\arrow["{p_A}", from=1-2, to=2-2]
			\arrow["\shortmid"{marking}, Rightarrow, no head, from=1-3, to=1-4]
			\arrow["{p_B}"', from=1-3, to=2-3]
			\arrow["{\pi_B}"{description}, draw=none, from=1-3, to=2-4]
			\arrow["{p_B}", from=1-4, to=2-4]
			\arrow["\shortmid"{marking}, Rightarrow, no head, from=2-1, to=2-2]
			\arrow["\shortmid"{marking}, Rightarrow, no head, from=2-3, to=2-4]
		\end{tikzcd}\]
	so that $f\circ p_A = g\circ p_B$, and terminal among all such. This means that
	given any loose morphism $u : U\pto V$, tight morphisms $A \xot a U \xto b B$ and $A \xot {a'} V \xto {b'} B$ and cells
	% https://q.uiver.app/#q=WzAsOCxbMCwwLCJYIl0sWzEsMCwiWSJdLFswLDEsIkEiXSxbMSwxLCJBIl0sWzIsMCwiWCJdLFszLDAsIlkiXSxbMiwxLCJCIl0sWzMsMSwiQiJdLFswLDEsInUiLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbMCwyLCJhIiwyXSxbMSwzLCJhJyJdLFsyLDMsIiIsMix7ImxldmVsIjoyLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs0LDUsInUiLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbNiw3LCIiLDIseyJsZXZlbCI6Miwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNCw2LCJiIiwyXSxbNSw3LCJiJyJdLFswLDMsIlxceGlfMSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs0LDcsIlxceGlfMiIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==
	\[\begin{tikzcd}[cramped]
			U & V & U & V \\
			A & A & B & B
			\arrow["u", "\shortmid"{marking}, from=1-1, to=1-2]
			\arrow["a"', from=1-1, to=2-1]
			\arrow["{\xi_A}"{description}, draw=none, from=1-1, to=2-2]
			\arrow["{a'}", from=1-2, to=2-2]
			\arrow["u", "\shortmid"{marking}, from=1-3, to=1-4]
			\arrow["b"', from=1-3, to=2-3]
			\arrow["{\xi_B}"{description}, draw=none, from=1-3, to=2-4]
			\arrow["{b'}", from=1-4, to=2-4]
			\arrow["\shortmid"{marking}, Rightarrow, no head, from=2-1, to=2-2]
			\arrow["\shortmid"{marking}, Rightarrow, no head, from=2-3, to=2-4]
		\end{tikzcd}\]
	such that $\frac{\xi_A}f = \frac{\xi_B}g$ (so in particular, $f\circ a = g\circ b$ and $f\circ a' = g\circ b'$),
	\begin{enumerate}
		\item there exists a unique pair of tight morphisms $\langle a,b\rangle : U\to A\times_X B$ and $\langle a',b'\rangle : V\to A\times_X B$, so that in particular $A\times_X B$ is a pullback in $\clD_0$;% (so, in particular, $p_A\circ\langle a,b\rangle = a$, $p_B\circ \langle a,b\rangle = b$, $p_A\circ \langle a',b'\rangle = a'$, $p_B\circ \langle a',b'\rangle = b'$);
		\item there exists a unique factorization of cells $\xi_A,\xi_B$ as %cell 
		      % https://q.uiver.app/#q=WzAsMTAsWzEsMSwiQVxcdGltZXNfWCBCIl0sWzMsMiwiQVxcdGltZXNfWCBCIl0sWzIsMSwiQSJdLFswLDIsIkIiXSxbMiwzLCJCIl0sWzQsMiwiQSJdLFsxLDMsIlgiXSxbMyw0LCJYIl0sWzEsMCwiVSJdLFszLDEsIlYiXSxbMCwzLCJwX0IiLDFdLFswLDJdLFsxLDQsInBfQiIsMV0sWzEsNSwicF9BIiwyXSxbMCwxLCIiLDEseyJsZXZlbCI6Miwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMyw2LCJnIiwyXSxbMiw2LCJmIiwyXSxbNCw3LCJnIl0sWzUsNywiZiJdLFszLDQsIiIsMSx7ImxldmVsIjoyLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs2LDcsIiIsMSx7ImxldmVsIjoyLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsyLDUsIiIsMSx7ImxldmVsIjoyLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFswLDYsIiIsMSx7InN0eWxlIjp7Im5hbWUiOiJjb3JuZXIifX1dLFsxLDcsIiIsMSx7InN0eWxlIjp7Im5hbWUiOiJjb3JuZXIifX1dLFs4LDMsIiIsMSx7ImN1cnZlIjoyfV0sWzgsMl0sWzksNV0sWzksNCwiIiwxLHsiY3VydmUiOjJ9XSxbOCw5LCJ1IiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fV0sWzgsMCwiISIsMCx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFs5LDEsIiEiLDIseyJsYWJlbF9wb3NpdGlvbiI6ODAsInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dXQ==
		      \[\begin{tikzcd}[cramped]
				      & U \\
				      & {A\times_X B} & A & V \\
				      B &&& {A\times_X B} & A \\
				      & X & B \\
				      &&& X
				      \arrow["{!}", dashed, from=1-2, to=2-2]
				      \arrow[from=1-2, to=2-3]
				      \arrow["u", "\shortmid"{marking}, from=1-2, to=2-4]
				      \arrow[curve={height=12pt}, from=1-2, to=3-1]
				      \arrow[from=2-2, to=2-3]
				      \arrow["{p_B}"{description}, from=2-2, to=3-1]
				      \arrow["\shortmid"{marking}, Rightarrow, no head, from=2-2, to=3-4]
				      \arrow["\lrcorner"{anchor=center, pos=0.125, rotate=-45}, draw=none, from=2-2, to=4-2]
				      \arrow["\shortmid"{marking}, Rightarrow, no head, from=2-3, to=3-5]
				      \arrow["f"', from=2-3, to=4-2]
				      \arrow["{!}"'{pos=0.8}, dashed, from=2-4, to=3-4]
				      \arrow[from=2-4, to=3-5]
				      \arrow[curve={height=12pt}, from=2-4, to=4-3]
				      \arrow["g"', from=3-1, to=4-2]
				      \arrow["\shortmid"{marking}, Rightarrow, no head, from=3-1, to=4-3]
				      \arrow["{p_A}"', from=3-4, to=3-5]
				      \arrow["{p_B}"{description}, from=3-4, to=4-3]
				      \arrow["\lrcorner"{anchor=center, pos=0.125, rotate=-45}, draw=none, from=3-4, to=5-4]
				      \arrow["f", from=3-5, to=5-4]
				      \arrow["\shortmid"{marking}, Rightarrow, no head, from=4-2, to=5-4]
				      \arrow["g", from=4-3, to=5-4]
			      \end{tikzcd}\]
		      through a unique mediating cell $\smallCell{u}{!}{!}{}[\langle \xi_A,\xi_B\rangle]$ such that
		      such that the equalities of cells $\xi_A = \frac{\langle \xi_A,\xi_B\rangle}{\pi_A}$ and $\xi_B = \frac{\langle \xi_A,\xi_B\rangle}{\pi_B}$ hold.
	\end{enumerate}
	The \emph{double pushout} of $A, B$ consists of the double product of $A,B$ in $\dblD^\vop$.
\end{definition}
\begin{definition}[Exponential of double categories]\label{exp_o_dbl}
	Let $\dblC,\dblD$ be two double categories; we construct the internal hom double category $\dblCat{[C,D]}$ as follows.
	\begin{itemize}
		\item The objects are pseudo double functors\footnote{A version $\dblCat{[C,D]}_\ell$ of this construction exists where objects are \emph{lax} double functors and the rest of the structure is unchanged --just, tight, loose morphisms and cells satisfy more coherence axioms. We do not need such generality as Walters et al. consider only \emph{pseudo} functors $\bbN \to\Sigma\clK$ in \cite{Katis1997}.} $F : \dblC \to\dblD$, as defined in \cite[3.5.1 and p. 145]{Grandis2019};
		\item tight morphisms $\phi : F \To G$ consist of families of tight morphisms $\phi_C : FC\to GC$ in $\dblD$ which are \emph{tightly natural}, i.e. for every tight $u : C\to C'$ one has $\phi_{C'}\circ Fu = Gu\circ \phi_C$, and \emph{loosely lax natural}, i.e. for every loose $c : C\pto C'$ there are cells $\smallCell{Fc}{\phi_C}{\phi_{C'}}{Gc}[\phi_c]$ such that
		      \begin{itemize}
			      \item the $\phi_c$ are compatible with the structure isomorphisms of $F,G$, i.e. with the loose isomorphisms $Fu\circ Fv \cong F(u\circ v)$, $\iota_{FC}\cong F(\iota_C)$, $Gu\circ Gv \cong G(u\circ v)$, $\iota_{GC}\cong G(\iota_C)$: for example, any time $c'\odot_h c : C \pto C' \pto C''$ are composable,
			            % https://q.uiver.app/#q=WzAsMTUsWzAsMCwiRkMiXSxbMSwwLCJGQyciXSxbMiwwLCJGQycnIl0sWzAsMSwiR0MiXSxbMSwxLCJHQyciXSxbMiwxLCJHQycnIl0sWzAsMiwiR0MiXSxbMiwyLCJHQycnIl0sWzQsMCwiRkMiXSxbNSwwLCJGQyciXSxbNiwwLCJGQycnIl0sWzQsMSwiRkMiXSxbNiwxLCJGQycnIl0sWzQsMiwiR0MiXSxbNiwyLCJHQycnIl0sWzAsMSwiRmMiLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbMSwyLCJGYyciLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbMyw0LCIiLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbNCw1LCIiLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbNiw3LCJHKGMnXFxvZG90X2ggYykiLDIseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbMCwzLCJcXHBoaV9DIiwyXSxbMSw0XSxbMiw1LCJcXHBoaV97QycnfSJdLFszLDYsIiIsMSx7ImxldmVsIjoyLCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzUsNywiIiwxLHsibGV2ZWwiOjIsInN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMyw3LCJcXGNvbmciLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMCw0LCJcXHBoaV9jIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzEsNSwiXFxwaGlfe2MnfSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs4LDksIkZjIiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fV0sWzksMTAsIkZjJyIsMCx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFsxMSwxMiwiIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fV0sWzEzLDE0LCJHKGMnXFxvZG90X2ggYykiLDIseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbOCwxMSwiIiwxLHsibGV2ZWwiOjIsInN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTAsMTIsIiIsMSx7ImxldmVsIjoyLCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzExLDEzLCJcXHBoaV9DIiwyXSxbMTIsMTQsIlxccGhpX3tDJyd9Il0sWzExLDE0LCJcXHBoaV97YydcXG9kb3RfaCBjfSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs4LDEyLCJcXGNvbmciLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMiwxMywiPSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==
			            \[\begin{tikzcd}[cramped]
					            FC & {FC'} & {FC''} && FC & {FC'} & {FC''} \\
					            GC & {GC'} & {GC''} && FC && {FC''} \\
					            GC && {GC''} && GC && {GC''}
					            \arrow["Fc", "\shortmid"{marking}, from=1-1, to=1-2]
					            \arrow["{\phi_C}"', from=1-1, to=2-1]
					            \arrow["{\phi_c}"{description}, draw=none, from=1-1, to=2-2]
					            \arrow["{Fc'}", "\shortmid"{marking}, from=1-2, to=1-3]
					            \arrow[from=1-2, to=2-2]
					            \arrow["{\phi_{c'}}"{description}, draw=none, from=1-2, to=2-3]
					            \arrow["{\phi_{C''}}", from=1-3, to=2-3]
					            \arrow["{=}"{description}, draw=none, from=1-3, to=3-5]
					            \arrow["Fc", "\shortmid"{marking}, from=1-5, to=1-6]
					            \arrow[Rightarrow, no head, from=1-5, to=2-5]
					            \arrow["\cong"{description}, draw=none, from=1-5, to=2-7]
					            \arrow["{Fc'}", "\shortmid"{marking}, from=1-6, to=1-7]
					            \arrow[Rightarrow, no head, from=1-7, to=2-7]
					            \arrow["\shortmid"{marking}, from=2-1, to=2-2]
					            \arrow[Rightarrow, no head, from=2-1, to=3-1]
					            \arrow["\cong"{description}, draw=none, from=2-1, to=3-3]
					            \arrow["\shortmid"{marking}, from=2-2, to=2-3]
					            \arrow[Rightarrow, no head, from=2-3, to=3-3]
					            \arrow["\shortmid"{marking}, from=2-5, to=2-7]
					            \arrow["{\phi_C}"', from=2-5, to=3-5]
					            \arrow["{\phi_{c'\odot_h c}}"{description}, draw=none, from=2-5, to=3-7]
					            \arrow["{\phi_{C''}}", from=2-7, to=3-7]
					            \arrow["{G(c'\odot_h c)}"', "\shortmid"{marking}, from=3-1, to=3-3]
					            \arrow["{G(c'\odot_h c)}"', "\shortmid"{marking}, from=3-5, to=3-7]
				            \end{tikzcd}\]
			      \item the $\phi_c$ are compatible with cells of $\dblD$, i.e. for every cell $\smallCell suvt[\zeta]$,
			            % https://q.uiver.app/#q=WzAsMTMsWzAsMCwiXFxidWxsZXQiXSxbMSwwLCJcXGJ1bGxldCJdLFsxLDEsIlxcYnVsbGV0Il0sWzAsMSwiXFxidWxsZXQiXSxbMCwyLCJcXGJ1bGxldCJdLFsxLDIsIlxcYnVsbGV0Il0sWzIsMSwiXFxlcXVpdiJdLFszLDAsIlxcYnVsbGV0Il0sWzMsMSwiXFxidWxsZXQiXSxbMywyLCJcXGJ1bGxldCJdLFs0LDAsIlxcYnVsbGV0Il0sWzQsMSwiXFxidWxsZXQiXSxbNCwyLCJcXGJ1bGxldCJdLFswLDEsIkZzIiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fV0sWzEsMiwiRnYiXSxbMCwzLCJGdSIsMl0sWzMsMiwiRnQiLDIseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbMyw0LCJcXHBoaV97XFwjfSIsMl0sWzQsNSwiR3QiLDIseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbMiw1LCJcXHBoaV97XFwjfSJdLFs3LDgsIlxccGhpX3tcXCN9IiwyXSxbOCw5LCJHdSIsMl0sWzEwLDExLCJcXHBoaV97XFwjfSJdLFsxMSwxMiwiR3YiXSxbNywxMCwiRnMiLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbOCwxMSwiIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fV0sWzksMTIsIkd0IiwyLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fV0sWzEzLDE2LCJGXFx6ZXRhIiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzE4LDE2LCJcXHBoaV90IiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzI0LDI1LCJcXHBoaV9zIiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzI2LDI1LCJHXFx6ZXRhIiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
			            \[\begin{tikzcd}[cramped]
					            {\cdot} & {\cdot} && {\cdot} & {\cdot} \\
					            {\cdot} & {\cdot} & \equiv & {\cdot} & {\cdot} \\
					            {\cdot} & {\cdot} && {\cdot} & {\cdot}
					            \arrow[""{name=0, anchor=center, inner sep=0}, "Fs", "\shortmid"{marking}, from=1-1, to=1-2]
					            \arrow["Fu"', from=1-1, to=2-1]
					            \arrow["Fv", from=1-2, to=2-2]
					            \arrow[""{name=1, anchor=center, inner sep=0}, "Fs", "\shortmid"{marking}, from=1-4, to=1-5]
					            \arrow["{\phi_{\#}}"', from=1-4, to=2-4]
					            \arrow["{\phi_{\#}}", from=1-5, to=2-5]
					            \arrow[""{name=2, anchor=center, inner sep=0}, "Ft"', "\shortmid"{marking}, from=2-1, to=2-2]
					            \arrow["{\phi_{\#}}"', from=2-1, to=3-1]
					            \arrow["{\phi_{\#}}", from=2-2, to=3-2]
					            \arrow[""{name=3, anchor=center, inner sep=0}, "\shortmid"{marking}, from=2-4, to=2-5]
					            \arrow["Gu"', from=2-4, to=3-4]
					            \arrow["Gv", from=2-5, to=3-5]
					            \arrow[""{name=4, anchor=center, inner sep=0}, "Gt"', "\shortmid"{marking}, from=3-1, to=3-2]
					            \arrow[""{name=5, anchor=center, inner sep=0}, "Gt"', "\shortmid"{marking}, from=3-4, to=3-5]
					            \arrow["{F\zeta}"{description}, draw=none, from=0, to=2]
					            \arrow["{\phi_s}"{description}, draw=none, from=1, to=3]
					            \arrow["{\phi_t}"{description}, draw=none, from=4, to=2]
					            \arrow["{G\zeta}"{description}, draw=none, from=5, to=3]
				            \end{tikzcd}\]
		      \end{itemize}
		\item loose morphisms $\psi : F\Loose G$ consist of
		      \begin{itemize}
			      \item families of loose morphisms $\psi_C : FC\pto GC$,
			      \item    cells of shape
			            % https://q.uiver.app/#q=WzAsNixbMCwwLCJGQyJdLFsxLDAsIkdDIl0sWzIsMCwiR0MnIl0sWzAsMSwiRkMiXSxbMSwxLCJGQyciXSxbMiwxLCJHQyciXSxbMCwxLCJcXHBzaV9DIiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fV0sWzAsMywiIiwwLHsibGV2ZWwiOjIsInN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMSwyLCJHYyIsMCx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFsyLDUsIiIsMCx7ImxldmVsIjoyLCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzMsNCwiRmMiLDIseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbNCw1LCJcXHBzaV97Qyd9IiwyLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fV0sWzEsNCwiXFxwc2lfYyIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==
			            \[\begin{tikzcd}[cramped]
					            FC & GC & {GC'} \\
					            FC & {FC'} & {GC'}
					            \arrow["{\psi_C}", "\shortmid"{marking}, from=1-1, to=1-2]
					            \arrow[Rightarrow, no head, from=1-1, to=2-1]
					            \arrow["Gc", "\shortmid"{marking}, from=1-2, to=1-3]
					            \arrow["{\psi_c}"{description}, draw=none, from=1-2, to=2-2]
					            \arrow[Rightarrow, no head, from=1-3, to=2-3]
					            \arrow["Fc"', "\shortmid"{marking}, from=2-1, to=2-2]
					            \arrow["{\psi_{C'}}"', "\shortmid"{marking}, from=2-2, to=2-3]
				            \end{tikzcd}\]
			      \item for each $u : C\to C'$ in $\dblC$, cells in $\dblD$ of shape
			            % https://q.uiver.app/#q=WzAsNCxbMCwwLCJGQyJdLFsxLDAsIkdDIl0sWzAsMSwiRkMnIl0sWzEsMSwiR0MnIl0sWzAsMSwiXFxwc2lfQyIsMCx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFswLDIsIkZmIiwyXSxbMSwzLCJHZiJdLFsyLDMsIlxccHNpX3tDJ30iLDIseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbNCw3LCJcXHBzaV9mIiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
			            \[\begin{tikzcd}[cramped]
					            FC & GC \\
					            {FC'} & {GC'}
					            \arrow[""{name=0, anchor=center, inner sep=0}, "{\psi_C}", "\shortmid"{marking}, from=1-1, to=1-2]
					            \arrow["Fu"', from=1-1, to=2-1]
					            \arrow["Gu", from=1-2, to=2-2]
					            \arrow[""{name=1, anchor=center, inner sep=0}, "{\psi_{C'}}"', "\shortmid"{marking}, from=2-1, to=2-2]
					            \arrow["{\psi_f}"{description}, draw=none, from=0, to=1]
				            \end{tikzcd}\]
		      \end{itemize}
		      such that for every cell $\smallCell sfgt[\zeta]$,
		      % https://q.uiver.app/#q=WzAsMTksWzAsMCwiXFxidWxsZXQiXSxbMSwwLCJcXGJ1bGxldCJdLFswLDEsIlxcYnVsbGV0Il0sWzEsMSwiXFxidWxsZXQiXSxbMiwwLCJcXGJ1bGxldCJdLFsyLDEsIlxcYnVsbGV0Il0sWzAsMiwiXFxidWxsZXQiXSxbMSwyLCJcXGJ1bGxldCJdLFsyLDIsIlxcYnVsbGV0Il0sWzMsMSwiXFxlcXVpdiJdLFs0LDAsIlxcYnVsbGV0Il0sWzQsMSwiXFxidWxsZXQiXSxbNCwyLCJcXGJ1bGxldCJdLFs1LDAsIlxcYnVsbGV0Il0sWzUsMSwiXFxidWxsZXQiXSxbNSwyLCJcXGJ1bGxldCJdLFs2LDAsIlxcYnVsbGV0Il0sWzYsMSwiXFxidWxsZXQiXSxbNiwyLCJcXGJ1bGxldCJdLFswLDEsIlxccHNpX3tcXCN9IiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fV0sWzAsMiwiRnUiLDJdLFsxLDNdLFsyLDMsIlxccHNpX3tcXCN9IiwyLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fV0sWzEsNCwiR3MiLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbMyw1LCJHdCIsMix7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFs0LDUsIkd2Il0sWzIsNiwiIiwwLHsibGV2ZWwiOjIsInN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNSw4LCIiLDAseyJsZXZlbCI6Miwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs2LDcsIkZ0IiwyLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fV0sWzcsOCwiXFxwc2lfe1xcI30iLDIseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbMyw3LCJcXHBzaV90IiwxLHsibGV2ZWwiOjIsInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxMCwxMSwiIiwxLHsibGV2ZWwiOjIsInN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTEsMTIsIkZ1IiwyXSxbMTQsMTVdLFsxNiwxNywiIiwxLHsibGV2ZWwiOjIsInN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTcsMTgsIkd2Il0sWzExLDE0LCJGcyIsMCx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFsxNCwxNywiIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fV0sWzEyLDE1LCJGdCIsMix7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFsxNSwxOCwiXFxwc2lfe1xcI30iLDIseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbMTAsMTMsIlxccHNpX3tcXCN9IiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fV0sWzEzLDE2LCJHcyIsMCx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFsxMywxNCwiXFxwc2lfcyIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxOSwyMiwiXFxwc2lfZiIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsyMywyNCwiR1xcemV0YSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFszNiwzOCwiRlxcemV0YSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFszNywzOSwiXFxwc2lfdiIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==
		      \[\begin{tikzcd}[cramped]
				      \cdot & \cdot & \cdot && \cdot & \cdot & \cdot \\
				      \cdot & \cdot & \cdot & \equiv & \cdot & \cdot & \cdot \\
				      \cdot & \cdot & \cdot && \cdot & \cdot & \cdot
				      \arrow[""{name=0, anchor=center, inner sep=0}, "{\psi_{\#}}", "\shortmid"{marking}, from=1-1, to=1-2]
				      \arrow["Fu"', from=1-1, to=2-1]
				      \arrow[""{name=1, anchor=center, inner sep=0}, "Gs", "\shortmid"{marking}, from=1-2, to=1-3]
				      \arrow[from=1-2, to=2-2]
				      \arrow["Gv", from=1-3, to=2-3]
				      \arrow["{\psi_{\#}}", "\shortmid"{marking}, from=1-5, to=1-6]
				      \arrow[Rightarrow, no head, from=1-5, to=2-5]
				      \arrow["Gs", "\shortmid"{marking}, from=1-6, to=1-7]
				      \arrow["{\psi_s}"{description}, draw=none, from=1-6, to=2-6]
				      \arrow[Rightarrow, no head, from=1-7, to=2-7]
				      \arrow[""{name=2, anchor=center, inner sep=0}, "{\psi_{\#}}"', "\shortmid"{marking}, from=2-1, to=2-2]
				      \arrow[Rightarrow, no head, from=2-1, to=3-1]
				      \arrow[""{name=3, anchor=center, inner sep=0}, "Gt"', "\shortmid"{marking}, from=2-2, to=2-3]
				      \arrow["{\psi_t}"{description}, draw=none, from=2-2, to=3-2]
				      \arrow[Rightarrow, no head, from=2-3, to=3-3]
				      \arrow[""{name=4, anchor=center, inner sep=0}, "Fs", "\shortmid"{marking}, from=2-5, to=2-6]
				      \arrow["Fu"', from=2-5, to=3-5]
				      \arrow[""{name=5, anchor=center, inner sep=0}, "\shortmid"{marking}, from=2-6, to=2-7]
				      \arrow[from=2-6, to=3-6]
				      \arrow["Gv", from=2-7, to=3-7]
				      \arrow["Ft"', "\shortmid"{marking}, from=3-1, to=3-2]
				      \arrow["{\psi_{\#}}"', "\shortmid"{marking}, from=3-2, to=3-3]
				      \arrow[""{name=6, anchor=center, inner sep=0}, "Ft"', "\shortmid"{marking}, from=3-5, to=3-6]
				      \arrow[""{name=7, anchor=center, inner sep=0}, "{\psi_{\#}}"', "\shortmid"{marking}, from=3-6, to=3-7]
				      \arrow["{\psi_f}"{description}, draw=none, from=0, to=2]
				      \arrow["{G\zeta}"{description}, draw=none, from=1, to=3]
				      \arrow["{F\zeta}"{description}, draw=none, from=4, to=6]
				      \arrow["{\psi_v}"{description}, draw=none, from=5, to=7]
			      \end{tikzcd}\]
		\item cells $\smallCell\psi\phi{\phi'}{\psi'}[\Delta]$ in $[\dblC,\dblD]$ consist of families $\Delta_C$ of cells of $\dblD$ indexed by the objects of $\dblC$,
		      % https://q.uiver.app/#q=WzAsNCxbMCwwLCJGIl0sWzEsMCwiRyJdLFswLDEsIkYnIl0sWzEsMSwiRyciXSxbMCwyLCJcXHBoaSIsMl0sWzIsMywiXFxwc2knIiwyLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fV0sWzAsMSwiXFxwc2kiLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbMSwzLCJcXHBoaSciXSxbNiw1LCJcXERlbHRhIiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
		      \[\begin{tikzcd}[cramped]
				      F & G \\
				      {F'} & {G'}
				      \arrow[""{name=0, anchor=center, inner sep=0}, "\psi", "\shortmid"{marking}, from=1-1, to=1-2]
				      \arrow["\phi"', from=1-1, to=2-1]
				      \arrow["{\phi'}", from=1-2, to=2-2]
				      \arrow[""{name=1, anchor=center, inner sep=0}, "{\psi'}"', "\shortmid"{marking}, from=2-1, to=2-2]
				      \arrow["\Delta"{description}, draw=none, from=0, to=1]
			      \end{tikzcd}\]
		      such that for every loose morphism $c : C\pto C'$ and tight morphism $f : C\to C'$, the following conditions are satisfied:
		      \begin{itemize}
			      \item compatibility with the $\psi_c$:
			            % https://q.uiver.app/#q=WzAsMTksWzAsMCwiRkMiXSxbMSwwLCJHQyJdLFsyLDAsIkdDJyJdLFswLDEsIkYnQyJdLFsxLDEsIkcnQyJdLFsyLDEsIkcnQyciXSxbMCwyLCJGJ0MiXSxbMSwyLCJGJ0MnIl0sWzIsMiwiRydDJyJdLFszLDEsIlxcZXF1aXYiXSxbNCwwLCJGQyJdLFs1LDAsIkdDIl0sWzYsMCwiR0MnIl0sWzQsMSwiRkMiXSxbNiwxLCJHQyciXSxbNSwxLCJGQyciXSxbNCwyLCJGJ0MiXSxbNSwyLCJGJ0MnIl0sWzYsMiwiRydDJyJdLFs1LDgsIiIsMCx7ImxldmVsIjoyLCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzMsNiwiIiwwLHsibGV2ZWwiOjIsInN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMCwzLCJcXHBoaV9DIiwyXSxbMyw0LCIiLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbNCw1LCIiLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbNiw3LCJGJ2MiLDIseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbNyw4LCJcXHBzaSdfe0MnfSIsMix7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFsxLDQsIlxccGhpJ19DIiwxXSxbMiw1LCJcXHBoaSdfe0MnfSJdLFswLDEsIlxccHNpX0MiLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbMSwyLCJHYyIsMCx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFswLDQsIlxcRGVsdGFfQyIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFszLDgsIlxccHNpJ19jIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzEsNSwiXFxwaGknX2MiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTAsMTEsIlxccHNpX0MiLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbMTEsMTIsIkdjIiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fV0sWzEzLDE1LCIiLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbMTUsMTQsIiIsMCx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFsxNiwxNywiRidjIiwyLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fV0sWzE3LDE4LCJcXHBzaSdfe0MnfSIsMix7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFsxNSwxNywiXFxwaGlfe0MnfSIsMV0sWzEwLDEzLCIiLDEseyJsZXZlbCI6Miwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxMiwxNCwiIiwxLHsibGV2ZWwiOjIsInN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTMsMTYsIlxccGhpX0MiLDJdLFsxNCwxOCwiXFxwaGknX3tDJ30iXSxbMTAsMTQsIlxccHNpX2MiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTUsMTgsIlxcRGVsdGFfe0MnfSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxMywxNywiXFxwaGlfYyIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==
			            \[\begin{tikzcd}[cramped]
					            FC & GC & {GC'} && FC & GC & {GC'} \\
					            {F'C} & {G'C} & {G'C'} & \equiv & FC & {FC'} & {GC'} \\
					            {F'C} & {F'C'} & {G'C'} && {F'C} & {F'C'} & {G'C'}
					            \arrow["{\psi_C}", "\shortmid"{marking}, from=1-1, to=1-2]
					            \arrow["{\phi_C}"', from=1-1, to=2-1]
					            \arrow["{\Delta_C}"{description}, draw=none, from=1-1, to=2-2]
					            \arrow["Gc", "\shortmid"{marking}, from=1-2, to=1-3]
					            \arrow["{\phi'_C}"{description}, from=1-2, to=2-2]
					            \arrow["{\phi'_c}"{description}, draw=none, from=1-2, to=2-3]
					            \arrow["{\phi'_{C'}}", from=1-3, to=2-3]
					            \arrow["{\psi_C}", "\shortmid"{marking}, from=1-5, to=1-6]
					            \arrow[Rightarrow, no head, from=1-5, to=2-5]
					            \arrow["{\psi_c}"{description}, draw=none, from=1-5, to=2-7]
					            \arrow["Gc", "\shortmid"{marking}, from=1-6, to=1-7]
					            \arrow[Rightarrow, no head, from=1-7, to=2-7]
					            \arrow["\shortmid"{marking}, from=2-1, to=2-2]
					            \arrow[Rightarrow, no head, from=2-1, to=3-1]
					            \arrow["{\psi'_c}"{description}, draw=none, from=2-1, to=3-3]
					            \arrow["\shortmid"{marking}, from=2-2, to=2-3]
					            \arrow[Rightarrow, no head, from=2-3, to=3-3]
					            \arrow["\shortmid"{marking}, from=2-5, to=2-6]
					            \arrow["{\phi_C}"', from=2-5, to=3-5]
					            \arrow["{\phi_c}"{description}, draw=none, from=2-5, to=3-6]
					            \arrow["\shortmid"{marking}, from=2-6, to=2-7]
					            \arrow["{\phi_{C'}}"{description}, from=2-6, to=3-6]
					            \arrow["{\Delta_{C'}}"{description}, draw=none, from=2-6, to=3-7]
					            \arrow["{\phi'_{C'}}", from=2-7, to=3-7]
					            \arrow["{F'c}"', "\shortmid"{marking}, from=3-1, to=3-2]
					            \arrow["{\psi'_{C'}}"', "\shortmid"{marking}, from=3-2, to=3-3]
					            \arrow["{F'c}"', "\shortmid"{marking}, from=3-5, to=3-6]
					            \arrow["{\psi'_{C'}}"', "\shortmid"{marking}, from=3-6, to=3-7]
				            \end{tikzcd}\]
			      \item compatibility with the $\psi_f$:
			            % https://q.uiver.app/#q=WzAsMTMsWzAsMCwiRkMiXSxbMSwwLCJHQyJdLFswLDEsIkZDJyJdLFsxLDEsIkdDJyJdLFswLDIsIkYnQyciXSxbMSwyLCJHJ0MnIl0sWzIsMSwiXFxlcXVpdiJdLFszLDAsIkZDIl0sWzQsMCwiR0MiXSxbMywxLCJGJ0MiXSxbNCwxLCJHJ0MiXSxbMywyLCJGJ0MnIl0sWzQsMiwiRydDJyJdLFswLDIsIkZ1IiwyXSxbMiw0LCJcXHBoaV97Qyd9IiwyXSxbNCw1LCJcXHBzaSdfe0MnfSIsMix7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFswLDEsIlxccHNpX0MiLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbMSwzLCJHdSJdLFszLDUsIlxccGhpJ197Qyd9Il0sWzIsMywiIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fV0sWzcsOSwiXFxwaGlfQyIsMl0sWzksMTEsIkYnZiIsMl0sWzExLDEyLCJcXHBzaSdfe0MnfSIsMix7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFsxMCwxMiwiRydmIl0sWzksMTAsIiIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFs4LDEwLCJcXHBoaSdfQyJdLFs3LDgsIlxccHNpX0MiLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbMCwzLCJcXHBzaV9mIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzIsNSwiXFxEZWx0YV97Qyd9IiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzcsMTAsIlxcRGVsdGFfQyIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs5LDEyLCJcXHBzaSdfZiIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==
			            \[\begin{tikzcd}[cramped]
					            FC & GC && FC & GC \\
					            {FC'} & {GC'} & \equiv & {F'C} & {G'C} \\
					            {F'C'} & {G'C'} && {F'C'} & {G'C'}
					            \arrow["{\psi_C}", "\shortmid"{marking}, from=1-1, to=1-2]
					            \arrow["Fu"', from=1-1, to=2-1]
					            \arrow["{\psi_f}"{description}, draw=none, from=1-1, to=2-2]
					            \arrow["Gu", from=1-2, to=2-2]
					            \arrow["{\psi_C}", "\shortmid"{marking}, from=1-4, to=1-5]
					            \arrow["{\phi_C}"', from=1-4, to=2-4]
					            \arrow["{\Delta_C}"{description}, draw=none, from=1-4, to=2-5]
					            \arrow["{\phi'_C}", from=1-5, to=2-5]
					            \arrow["\shortmid"{marking}, from=2-1, to=2-2]
					            \arrow["{\phi_{C'}}"', from=2-1, to=3-1]
					            \arrow["{\Delta_{C'}}"{description}, draw=none, from=2-1, to=3-2]
					            \arrow["{\phi'_{C'}}", from=2-2, to=3-2]
					            \arrow["\shortmid"{marking}, from=2-4, to=2-5]
					            \arrow["{F'f}"', from=2-4, to=3-4]
					            \arrow["{\psi'_f}"{description}, draw=none, from=2-4, to=3-5]
					            \arrow["{G'f}", from=2-5, to=3-5]
					            \arrow["{\psi'_{C'}}"', "\shortmid"{marking}, from=3-1, to=3-2]
					            \arrow["{\psi'_{C'}}"', "\shortmid"{marking}, from=3-4, to=3-5]
				            \end{tikzcd}\]
		      \end{itemize}
	\end{itemize}
\end{definition}
\begin{definition}[Tight monad morphism]
	\label{mormonad_tig}
	Let $(M : A\pto A,\mu,\eta)$, $(N : B\pto B,\nu,\gamma)$ be two monads on objects $A,B$, in a \PDC $\dblD$; a \emph{(tight) monad morphism} consists of a pair $(f,\alpha)$ where $f : A\to B$ is a tight morphism, and $\alpha$ a cell
	% https://q.uiver.app/#q=WzAsNCxbMCwwLCJBIl0sWzEsMCwiQSJdLFswLDEsIkIiXSxbMSwxLCJCIl0sWzAsMSwiTSIsMCx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFsyLDMsIk4iLDIseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbMCwyLCJmIiwyXSxbMSwzLCJmIl0sWzAsMywiXFxhbHBoYSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==
	\[\begin{tikzcd}[cramped]
			A & A \\
			B & B
			\arrow["M", "\shortmid"{marking}, from=1-1, to=1-2]
			\arrow["f"', from=1-1, to=2-1]
			\arrow["\alpha"{description}, draw=none, from=1-1, to=2-2]
			\arrow["f", from=1-2, to=2-2]
			\arrow["N"', "\shortmid"{marking}, from=2-1, to=2-2]
		\end{tikzcd}\]
	compatible with the monad structure of $M,N$ in the sense that $\frac\mu\alpha = \frac{\alpha\mid\alpha}{\nu}$ and $\frac\eta\alpha = \frac f\gamma$.
\end{definition}
This definition is used twice in the above discussion:
\begin{itemize}
	\item In \autoref{dgaddaaa}, every monad morphism in this sense	induces a monoid homomorphism $f\times\alpha : E\bowtie_M A^* \to B^*\bowtie_N E'$ through $f : A\to B$ and $\alpha : E\to E'$ (the carriers of $M$ and $N$ respectively).
	\item In \autoref{coro_fremonad}, a cell of type $\smallCell F{}{}N[\gamma]$ extends to a morphism of monads $\smallCell {M(F)}{}{}N[\gamma^*]$ promoting the construction outlined in \autoref{coro_fremonad} to a double functor.
\end{itemize}
\begin{definition}[Loose adjunction]\label{def_loose_adja}
	Two loose morphisms $l : A\pto B$, $r : B\pto A$ form a \emph{loose adjunction} in a \PDC $\dblD$ if they are equipped with
	\begin{itemize}
		\item two cells (called \emph{unit} and \emph{counit}),
		      % https://q.uiver.app/#q=WzAsOCxbMCwwLCJBIl0sWzEsMCwiQSJdLFswLDEsIkEiXSxbMSwxLCJBIl0sWzIsMCwiQiJdLFszLDAsIkIiXSxbMiwxLCJCIl0sWzMsMSwiQiJdLFsyLDMsInJcXGhvckMgbCIsMix7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFswLDIsIiIsMix7ImxldmVsIjoyLCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzEsMywiIiwwLHsibGV2ZWwiOjIsInN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMCwxLCIiLDAseyJsZXZlbCI6Miwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNiw3LCIiLDAseyJsZXZlbCI6Miwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNCw1LCJsXFxob3JDIHIiLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbNCw2LCIiLDEseyJsZXZlbCI6Miwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs1LDcsIiIsMSx7ImxldmVsIjoyLCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzAsMywiXFxldGEiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNCw3LCJcXGVwc2lsb24iLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XV0=
		      \[\begin{tikzcd}[cramped]
				      A & A & B & B \\
				      A & A & B & B
				      \arrow["\shortmid"{marking}, Rightarrow, no head, from=1-1, to=1-2]
				      \arrow[Rightarrow, no head, from=1-1, to=2-1]
				      \arrow["\eta"{description}, draw=none, from=1-1, to=2-2]
				      \arrow[Rightarrow, no head, from=1-2, to=2-2]
				      \arrow["{l\horC r}", "\shortmid"{marking}, from=1-3, to=1-4]
				      \arrow[Rightarrow, no head, from=1-3, to=2-3]
				      \arrow["\epsilon"{description}, draw=none, from=1-3, to=2-4]
				      \arrow[Rightarrow, no head, from=1-4, to=2-4]
				      \arrow["{r\horC l}"', "\shortmid"{marking}, from=2-1, to=2-2]
				      \arrow["\shortmid"{marking}, Rightarrow, no head, from=2-3, to=2-4]
			      \end{tikzcd}\]
		\item satisfying the adjunction identities $l = \frac{\eta\mid l}{l\mid\epsilon}$ and $r = \frac{r\mid \eta}{\epsilon\mid r}$.
	\end{itemize}
\end{definition}
\subsection{Proofs}
\begin{savvyProof}[Proof of \autoref{crucial_thm}.]
	Unpacking the definition of algebra for the monad $M=((E,\langle d,s\rangle) : A \pto A,\eta,\mu)$ as in \autoref{sgrulbio}, when instantiated in $\cartDblMly$, we get
	\begin{enumtag}{ad}
		\item a Mealy automaton $(P,\langle \delta,\sigma\rangle) : A\times P \to P\times X$;% (with slight abuse of notation, we denote $P$ the state space of the automaton);
		\item an algebra map $\xi : E \times P \to P$ defining a cell
		\[\begin{tikzcd}[cramped, ampersand replacement=\&]
				A \& A \& X \\
				A \&\& X
				\arrow["M", "\shortmid"{marking}, from=1-1, to=1-2]
				\arrow[Rightarrow, no head, from=1-1, to=2-1]
				\arrow["\xi"{description}, draw=none, from=1-1, to=2-3]
				\arrow["P", "\shortmid"{marking}, from=1-2, to=1-3]
				\arrow[Rightarrow, no head, from=1-3, to=2-3]
				\arrow["P"', "\shortmid"{marking}, from=2-1, to=2-3]
			\end{tikzcd}\]
	\end{enumtag}
	subject to the following conditions (the notation is as in \autoref{deffa_monada}):
	\begin{enumtag}{ax}
		\item \label{ax_1} cell axiom for $\xi$, I: for all $x\in X, t\in P, e\in E$ we have $\sigma (a , \xi (e , x)) = \sigma (a \sact e , x)$;
		\item \label{ax_2} cell axiom for $\xi$, II: for all $x\in X, t\in P, e\in E$ we have $\delta (a , \xi (e , x)) = \xi (a \dact e , \delta (a \sact e , x))$;
		\item \label{ax_3} unitality: for all $t\in P$ we have $\xi (e_0 , x) = x$ %$\xi (t , e_0) = t$;
		\item \label{ax_4} associativity: for $t\in P$, $e,e'\in E$ we have $\xi (\mu (e , e') , x) = \xi (e , \xi (e' , x))$ %$\xi (\xi (t , e) , e') = \xi (t , \mu (e , e'))$.
	\end{enumtag}
	Denote for convenience $\xi(t,e)$ as $t \centerdot e$; then \ref{ax_3} and \ref{ax_4} are the axioms
	\[\label{action_ofE}\forall t : e_0 \centerdot t = t \qquad\qquad \forall t,e,e' : (e \cdot e')\centerdot t = e\centerdot(e'\centerdot t)\]
	of a left action of $(E,\cdot,e_0)$ on $P$.

	In this notation, axioms \ref{ax_1} and \ref{ax_2} read
	\[
		\sigma (a , e \centerdot t) = \sigma (a \sact e , t)\qquad\qquad
		\delta (a , e \centerdot t) = (a \dact e) \centerdot (\delta (a \sact e , t))
	\]
	the first of which asserts the fact that $\sigma : A\times P \to X$ is `balanced' with respect to the structure of left $E$-sets on $(P,\centerdot),(A,\sact)$ (as a consequence, $\sigma$ descends to a map from the tensor product of $E$-sets $\hat\sigma : A\otimes_E P \to X$). As for the second, this is precisely the condition stated in \autoref{crucialemma} ensuring that the two actions of $A^*$ (induced by $\delta$) and $E$ (in \eqref{action_ofE}) on $P$ match to an action of $E\bowtie A^*$.
\end{savvyProof}
\begin{savvyProof}[Proof of \autoref{coprod_no}]
	The non existence of an initial object follows from \autoref{a_trick}; such an object corresponds to a unique cell $u_F$ so that the square
	% https://q.uiver.app/#q=WzAsNCxbMCwxLCJBXFx0aW1lcyBFIl0sWzEsMSwiRVxcdGltZXMgQiJdLFswLDAsIlxcZW1wdHlcXHRpbWVzIDEiXSxbMSwwLCIxXFx0aW1lcyBcXGVtcHR5Il0sWzIsMCwiIVxcdGltZXMgZV8wIiwyXSxbMCwxXSxbMywxLCJlXzBcXHRpbWVzICEiXSxbMiwzXV0=
	\[\begin{tikzcd}[cramped, ampersand replacement=\&]
			{\empty\times 1} \& {1\times \empty} \\
			{A\times E} \& {E\times B}
			\arrow[from=1-1, to=1-2]
			\arrow["{!\times e_0}"', from=1-1, to=2-1]
			\arrow["{e_0\times !}", from=1-2, to=2-2]
			\arrow[from=2-1, to=2-2]
		\end{tikzcd}\]
	commutes; this forces $E$ to be a singleton. For a similar reason, just a little bit more convoluted to enforce, coproducts, in the sense of \autoref{def_procopro_pc} (see also \cite{Grandis1999}) do not exist.
\end{savvyProof}
\begin{savvyProof}[Proof of \autoref{has_cumpa}]
	We build the companion of $f : A\to B$ as a cell
	% https://q.uiver.app/#q=WzAsNCxbMCwwLCJBXFx0aW1lcyAxIl0sWzEsMCwiQSJdLFsyLDAsIkIiXSxbMywwLCIxXFx0aW1lcyBCIl0sWzAsMSwiXFxzaW0iXSxbMSwyLCJmIl0sWzIsMywiXFxzaW0iXV0=
	\[\begin{tikzcd}[cramped, ampersand replacement=\&]
			{A\times 1} \& A \& B \& {1\times B}
			\arrow["\sim", from=1-1, to=1-2]
			\arrow["f", from=1-2, to=1-3]
			\arrow["\sim", from=1-3, to=1-4]
		\end{tikzcd}\]
	for which the `unit' and `counit' cells, boiling down to the diagrams
	% https://q.uiver.app/#q=WzAsMTIsWzAsMCwiQVxcdGltZXMgMSJdLFsxLDAsIkEiXSxbMiwwLCJCIl0sWzMsMCwiMVxcdGltZXMgQiJdLFswLDEsIkJcXHRpbWVzIDEiXSxbMywxLCIxXFx0aW1lcyBCIl0sWzQsMSwiQVxcdGltZXMgMSJdLFs1LDEsIkEiXSxbNiwxLCJCIl0sWzcsMSwiMVxcdGltZXMgQiJdLFs3LDAsIjFcXHRpbWVzIEEiXSxbNCwwLCJBXFx0aW1lcyAxIl0sWzAsMSwiXFxzaW0iXSxbMSwyLCJmIl0sWzIsMywiXFxzaW0iXSxbMyw1LCIiLDAseyJsZXZlbCI6Miwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs0LDUsIiIsMix7ImxldmVsIjoyLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFswLDQsImZcXHRpbWVzIDEiLDJdLFs2LDcsIlxcc2ltIiwyXSxbNyw4LCJmIiwyXSxbOCw5LCJcXHNpbSIsMl0sWzEwLDksIjFcXHRpbWVzIGYiXSxbMTEsNiwiIiwyLHsibGV2ZWwiOjIsInN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTEsMTAsIiIsMCx7ImxldmVsIjoyLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==
	\[\begin{tikzcd}[cramped, ampersand replacement=\&]
			{A\times 1} \& A \& B \& {1\times B} \& {A\times 1} \&\&\& {1\times A} \\
			{B\times 1} \&\&\& {1\times B} \& {A\times 1} \& A \& B \& {1\times B,}
			\arrow["\sim", from=1-1, to=1-2]
			\arrow["{f\times 1}"', from=1-1, to=2-1]
			\arrow["f", from=1-2, to=1-3]
			\arrow["\sim", from=1-3, to=1-4]
			\arrow[Rightarrow, no head, from=1-4, to=2-4]
			\arrow["\shortmid"{marking}, Rightarrow, no head, from=1-5, to=1-8]
			\arrow[Rightarrow, no head, from=1-5, to=2-5]
			\arrow["{1\times f}", from=1-8, to=2-8]
			\arrow["\shortmid"{marking}, Rightarrow, no head, from=2-1, to=2-4]
			\arrow["\sim"', from=2-5, to=2-6]
			\arrow["f"', from=2-6, to=2-7]
			\arrow["\sim"', from=2-7, to=2-8]
		\end{tikzcd}\]
	are readily constructed; the zig and zag identities are also totally elementary.
\end{savvyProof}
\begin{proof}[Proof of \autoref{crucialemma}]
	From \autoref{sbriggosbraggo}, $H\bowtie G$ comes equipped with a universal choice of a cospan $H \xto{i_H}H\bowtie G\xot{i_G} G$; precomposing a left representation $H\bowtie G \to\Set$ with $i_H, i_G$ induces a pair of left representations $H \to\Set, G\to\Set$ subject to condition \eqref{gndgoadbgoadb}, as it can be immediately seen from the relation $(1,g)\bullet (h,1) = (g\dact h,g\sact h)$ present in $H\bowtie G$.

	Conversely, given two representations $\alpha,\beta$ satisfying \eqref{gndgoadbgoadb}, we just have to show that posing $(h,g)\bullet x := \alpha(h, \beta(g,x))$ defines an action of $H\bowtie G$. The fact that $(1,1)\star x = x$ is immediate. As for associativity, one easily finds that
	\begin{align*}
		\big((h,g)\bullet (h',g')\big)\star x & = (h . g\dact h , g \sact h . g') \star x                      \\
		                                      & =\alpha(h . g\dact h , \beta(g \sact h . g',x) )               \\
		                                      & =\alpha(h, \alpha(g\dact h , \beta(g \sact h \beta(g',x) ) ) ) \\
		                                      & =\alpha(h, \beta(g , \alpha(h', \beta(g',x))))                 \\
		                                      & =\alpha(h, \beta(g , (h',g')\star x))                          \\
		                                      & =(h,g) \star ((h',g')\star x)
	\end{align*}
	which concludes the proof.
\end{proof}
